The 2024 Brain Tumor Segmentation (BraTS) Challenge: Glioma Segmentation on Post-treatment MRI

Gliomas are the most common malignant primary brain tumors in adults and one of the deadliest types of cancer. There are many challenges in treatment and monitoring due to the genetic diversity and high intrinsic heterogeneity in appearance, shape, histology, and treatment response. Treatments include surgery, radiation, and systemic therapies, with magnetic resonance imaging (MRI) playing a key role in treatment planning and post-treatment longitudinal assessment. The 2024 Brain Tumor Segmentation (BraTS) challenge on post-treatment glioma MRI will provide a community standard and benchmark for state-of-the-art automated segmentation models based on the largest expert-annotated post-treatment glioma MRI dataset. Challenge competitors will develop automated segmentation models to predict four distinct tumor sub-regions consisting of enhancing tissue (ET), surrounding non-enhancing T2/fluid-attenuated inversion recovery (FLAIR) hyperintensity (SNFH), non-enhancing tumor core (NETC), and resection cavity (RC). Models will be evaluated on separate validation and test datasets using standardized performance metrics utilized across the BraTS 2024 cluster of challenges, including lesion-wise Dice Similarity Coefficient and Hausdorff Distance. Models developed during this challenge will advance the field of automated MRI segmentation and contribute to their integration into clinical practice, ultimately enhancing patient care.

==> Notes.tex <==
# Important notes/TODO for manuscript goes here 

Please make sure you add the following authors in the next revision of each challenge manuscript.
Verena Chung, Sage Bionetworks
Maria Diaz, Sage Bionetworks
Byrone Cole, Sage Bionetworks
James Eddy, Sage BIonetworks
Jake Albrecht, Sage Bionetworks

It would also be nice to have a consistent description of the Synapse platform: 

Synapse is a collaborative research platform that helps teams share, organize, and discuss their scientific research.  Synapse supports the capacity to create and manage community data challenges, using containerized models for secure evaluation of participant submitted methods.

 
